A Graph Convolutional Network Composition Framework for Semi-supervised Classification

Graph convolutional networks (GCNs) have gained popularity due to high performance achievable on several downstream tasks including node classification. Several architectural variants of these networks have been proposed and investigated with experimental studies in the literature. Motivated by a recent work on simplifying GCNs, we study the problem of designing other variants and propose a framework to compose networks using building blocks of GCN. The framework offers flexibility to compose and evaluate different networks using feature and/or label propagation networks, linear or non-linear networks, with each composition having different computational complexity. We conduct a detailed experimental study on several benchmark datasets with many variants and present observations from our evaluation. Our empirical experimental results suggest that several newly composed variants are useful alternatives to consider because they are as competitive as, or better than the original GCN.

==> sections/baselines_exp_setup.tex <==
 \indent\textbf{Baselines}
We evaluate our composed models against feature propagation based models like GCN \cite{gcn} and its corresponding simplified linear version, SGCN \cite{sgcn}. We also include LPNN \cite{lpnn} from the label propagation regime as another baseline. We only consider LPNN as it was shown to be superior than LPA\todo{cite} and EmbedNN \cite{embednn} in \cite{lpnn}. LPNN encodes local continuity through $f$  while also utilizing the node features through $g$. It is worthwhile to note that our label propagation variants aggregates the probabilities, while in LPNN, label propagation is loosely used as a regularizer\todo{Is it an accurate statement?}. Our implementation of LPNN jointly optimizes the following loss formulation, 
\begin{multline}
    \mu_{G} Tr\{f^{T}(I_{N}-S)f\} + \mu_{l} \sum_{i=1}^{l}\norm{f_{i}-y_{i}}^{2} + \mu_{u}\sum_{i=l+1}^{n}\norm{f_{i}}^{2} + 
    \lambda_{l} \sum_{i=1}^{l} \textrm{KL}(y_{i}||g_{i})\\ + \lambda_{u} \sum_{i=l+1}^{n} \textrm{KL}(f_{i}||g_{i})
\end{multline}  
\indent\textbf{Training Specifications}
All baselines and composed models were implemented and the evaluated in an identical setup. Each model was trained for 500 epochs with an early stopping criterion of no improvement in validation accuracy for 25 epochs. We used Adam optimizer to minimize the standard cross entropy loss for all the models (except LPNN). Hyper-parameter search was done using \textit{optuna} \cite{optuna}. For each dataset split, we swept through 2000 configurations using TPE sampler in \textit{optuna}. We computed test accuracy for the model configuration that achieves the maximum validation accuracy. 
{ 
    \setlength{\tabcolsep}{12pt}
    \begin{table}[]
        \centering
        \label{tab:hyp_table}
        \resizebox{\textwidth}{!}{
            \begin{tabular}{|c|c|c|}
                \hline
                \textbf{Hyperparamters} & \textbf{Search Space} & \textbf{Models} \\ \hline
            
                \begin{tabular}[c]{@{}c@{}}
                    learning rate, dropout, \\ weight decay\end{tabular} & uniform in (0,1) &  All \\ 
            
                \hline
            
                hidden dimensions &  [8, 16, 32, 64, 128] &  \begin{tabular}[c]{@{}c@{}}MLP based models, \\ GCN, LPGCN\end{tabular} \\ \hline
            
                \begin{tabular}[c]{@{}c@{}}$\mu_{G}$, $\mu_{l}$, $\mu_{u}$, \\ $\lambda_{l}$, $\lambda_{u}$\end{tabular} &  uniform in (0,1) &  LPNN \\ \hline
            \end{tabular}%
        }
    \end{table}
}

In our set of experiments we consider one hidden layer for MLP, two convolutional layers for GCN and k in $S^{k}$ for SGCN is set to two. For LPNN, $h^b()$ and $g(f,x)$ consists of 2 hidden layers of dimensions 128 and 64 as specified in \cite{lpnn}. We also set $h^a(.)$ to an identity function.  



==> sections/experiments_discussion.tex <==
\subsubsection{Datasets}
\begin{dataset_description}
We evaluate on five datasets: Cora, Citeseer, Pubmed taken from~\cite{ica}, and ACM, DBLP taken from~\cite{han}.\\
\indent\textbf{Cora.} The Cora dataset consists of Machine Learning papers represented as nodes. Two nodes are connected by an edge if they share a citation. Every node has a corresponding sparse binary bag-of-words representation of unique keywords. Each node can be classified into one of the following seven classes: \textit{Case Based}, \textit{Genetic Algorithms}, \textit{Neural Networks}, \textit{Probabilistic Methods}, \textit{Reinforcement Learning}, \textit{Rule Learning}, and \textit{Theory}~\cite{ica}.\\ 
\indent\textbf{Citeseer.} The Citeseer dataset consists of scientific papers represented as nodes. Nodes are connected by citation links. Every node is described by a sparse binary word vector indicating the absence/presence of the corresponding keyword. Each node can be classified into one of the following six classes: \textit{Agents}, \textit{Artificial Intelligence}, \textit{Databases}, \textit{Information Retrieval}, \textit{Machine Learning}, and \textit{Human Computer Interaction}~\cite{ica}.\\
\indent\textbf{PubMed.} The PubMed dataset consists of scientific papers corresponding to diabetes from PubMed database, which are represented as nodes. Nodes are connected by citation links. Every node is described by a TF/IDF weighted word vector from a dictionary which consists of unique keywords. Each node can be classified into one of the following three classes: \textit{Diabetes Mellitus, Experimental}, \textit{Diabetes Mellitus Type 1}, \textit{Diabetes Mellitus Type 2}~\cite{ica}.\\
\indent\textbf{ACM.} The ACM dataset consists of scientific papers published in KDD, SIGMOD, SIGCOMM, MobiCOMM, and VLDB conferences. These papers are represented as nodes. An edge exists between two nodes if they share an author. Node features correspond to sparse binary bag-of-words representation of unique keywords. Each node can be classified into one of the following three classes: \textit{Database}, \textit{Wireless Communication}, and \textit{Data Mining}~\cite{han}.\\
\indent\textbf{DBLP.} The DBLP dataset consists of authors, who are represented as nodes. An edge exists between two nodes if they share a paper. Node features correspond to sparse binary bag-of-words representation of unique keywords. Each node can be classified into one of the following four classes: \textit{database}, \textit{data mining}, \textit{machine learning}, and \textit{information retrieval}~\cite{han}.
The detailed statistics of the datasets are tabulated in Table 2.
\begin{dataset_table}
    \begin{table}[]
    \centering
    \caption{Datasets Statistics}
    \label{tab:cv_main_few}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    \textbf{} & \textbf{Cora} & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{ACM} & \textbf{DBLP} \\ \hline
    \textbf{Nodes}         & 2,708 & 3,327 & 19,717 & 3,025 & 4,057 \\ \hline
    \textbf{Edges}        & 5,278 & 4,552 & 44,324 & 16,153 & 7,585 \\ \hline
    \textbf{Features} & 1,433 & 3,703 & 500 & 1,830 & 334 \\ \hline
    \textbf{Classes}     & 7 & 6 & 3 & 3 & 4 \\ \hline
    \textbf{Train Samples}      & 140/1208 & 120/1827 & 60/18217 & 60/1525 & 80/2557 \\ \hline 
    \textbf{Val Samples}    & 500 & 500 & 500 & 500 & 500 \\ \hline
    \textbf{Test Samples} & 1000 & 1000 & 1000 & 1000 & 1000 \\ \hline
    \end{tabular}%
    }
    \end{table}
\end{dataset_table}
\\Literature models evaluate on a standard split of the above mentioned datasets. A single split offers limited information about generalization performance of the classification models. To address this, we evaluate on standard data split as well as 10 random splits with both standard data split size and increasing training labels. We study model behavior under varying training data size. 

% \begin{algorithm}
% 	\State Repeat 5 times
% 	\begin{algorithmic}[1]
% 	    \State Get StratfiedKFold of the dataset with 2 splits
% 		\For {\texttt{train\_set}, \texttt{test\_set} in each split}
% 			\State \texttt{Test\_set} = uniform random sample 1000 nodes from \texttt{test\_set}
% 			\State \texttt{Validation\_set} = uniform random sample 500 nodes from \texttt{train\_set}
% 			\State \texttt{Train\_set} =  Uniform random sample 20 nodes per class from                       \texttt{train\_set}-\texttt{Validation\_set}
% 	\end{algorithmic} 
% \end{algorithm}
\end{dataset_description}


